Distributed Power Splitting for SWIPT in Relay Interference Channels using Game Theory

In this paper, we consider simultaneous wireless information and power transfer (SWIPT) in relay interference channels, where multiple source-destination pairs communicate through their dedicated energy harvesting relays. Each relay needs to split its received signal from sources into two streams: one for information forwarding and the other for energy harvesting. We develop a distributed power splitting framework using game theory to derive a profile of power splitting ratios for all relays that can achieve a good network-wide performance. Specifically, non-cooperative games are respectively formulated for pure amplify-and-forward (AF) and decode-and-forward (DF) networks, in which each link is modeled as a strategic player who aims to maximize its own achievable rate. The existence and uniqueness for the Nash equilibriums (NEs) of the formulated games are analyzed and a distributed algorithm with provable convergence to achieve the NEs is also developed. Subsequently, the developed framework is extended to the more general network setting with mixed AF and DF relays. All the theoretical analyses are validated by extensive numerical results. Simulation results show that the proposed game-theoretical approach can achieve a near-optimal network-wide performance on average, especially for the scenarios with relatively low and moderate interference.

==> power_splitting_AF_network.tex <==
\section{Distributed Power Splitting Scheme for Pure AF Network}\label{sec:Pure_AF_Network}
In this section, we focus on the the design of distributed power splitting scheme for the pure AF network, where all the relay nodes employ the AF relaying protocol. To choose an efficient profile of the power splitting ratios (i.e, $\pmb \rho$) that can achieve a good network-wide performance, the most direct way is to solve the following network utility maximization problem:
\begin{equation}\label{eq:cnetralized_optimization_AF}
\begin{array}{l}
 \mathop {\max }\limits_{\pmb \rho}  \sum\nolimits_{i = 1}^N {u_i^{AF}\left( {\pmb \rho}  \right)}  \\
 ~~~{\rm {s.t.}}\;\;\rho  \in {\mathcal A} \\
\end{array},
\end{equation}
where ${{u_i^{AF}}\left( {\pmb \rho}  \right)}$ is defined in (\ref{eq: utiliy_AF}), and ${\mathcal A} = \left\{ {\left. {\pmb \rho}  \right|0 \le {\rho _i} \le 1,\;\forall i \in {\mathcal N}} \right\}$ is the feasible set of ${\pmb \rho}$.

However, it can be easily checked that the optimization problem in (\ref{eq:cnetralized_optimization_AF}) is not convex. This means that the global optimal solution of (\ref{eq:cnetralized_optimization_AF}) cannot be efficiently achieved even in a centralized fashion, needless to say the heavy signaling overhead required by the centralized method. Motivated by this issue, we consider that all links are selfish and they aim to maximize their individual achievable rate by choosing their own power splitting ratio. Mathematically, this will involve the $i$th link solving the following optimization problem
\begin{equation}\label{eq:distributed_optimization_AF}
\begin{array}{l}
\mathop {\max }\limits_{{\rho _i}} \;\;\;{u_i^{AF}}\left( {{\rho _i},{\pmb \rho _{ - i}}} \right) = \frac{1}{2}\log \left( {1 + \gamma _i^{AF}} \right)\\
~~~~~~~~~~~~~~{\rm{s.t.}}\;\;\;{\rho _i} \in {{\mathcal A}_i}
\end{array},
\end{equation}
where ${{\pmb \rho} _{ - i}} = {\left[ {{\rho _1}, \ldots ,{\rho _{i - 1}},{\rho _{i + 1}}, \ldots {\rho _N}} \right]^T}$ denotes the vector of all links' power splitting ratios, except the $i$th one, and ${\cal A}_i = \left\{ {\left. \rho_i  \right|0 \le {\rho _i} \le 1} \right\}$ is the feasible set of the $i$th link's power splitting ratio.

We can observe from (\ref{eq:distributed_optimization_AF}) that the optimization problem to be solved by each link is coupled together due to the mutual interference over two hops. Thus, we can model the considered power splitting problem to be a non-cooperative game in game theory \cite{Fudenberg_Game_book}. Rooted in economics, game theory has lately become a popular tool in the design of competitive resource allocation algorithms in communication area \cite{Attar_JSAC_2012,Jorswieck_JSTSP_2012}.
Particularly, the considered power splitting problem can be modeled by the following non-cooperative game:
\begin{itemize}
\item \emph{{Players}}: The $N$ S-R-D links.
\item \emph{{Actions}}: Each link determines its power splitting ratio $\rho_i \in {\mathcal{A}}_i$ to maximize the achievable rate for its own link.
\item \emph{{Utilities}}: The achievable rate ${u_i^{AF}}\left( {{\rho _i},{\pmb \rho _{ - i}}} \right)$ defined in (\ref{eq: utiliy_AF}).
\end{itemize}

For convenience, we denote the formulated non-cooperative game as
\begin{equation}\label{eq:AF_game}
{\mathcal{G}}_{AF} = \left\langle {\mathcal{N},\left\{ \mathcal{A}_i  \right\},\left\{{{u}_i^{AF}}\left( {{\rho_i},{{{\pmb \rho}}_{ -i}}} \right)\right\} }\right\rangle.
\end{equation}

%\subsection{Solution of the Formulated Game}
The most well-known solution to the non-cooperative games is the (pure strategy) Nash equilibrium (NE). A NE of a given non-cooperative game $\left\langle  {{\cal N},\{ {{\bf{{\cal Q}}}_n}\} ,\left\{ {{{\cal U}_n}\left( {{{\bf{x}}_n},{{\bf{x}}_{ - n}}} \right)} \right\}} \right\rangle $ is a feasible point ${\bf{x}}^*$ such that
\begin{equation}
{\mathcal U}\left( {{\bf{x}}_n^*,{\bf{x}}_{ - n}^*} \right) \ge {\mathcal U}\left( {{{\bf{x}}_n},{\bf{x}}_{ - n}^*} \right),\;\forall {{\bf{x}}_n} \in {{\mathcal Q}_n}.
\end{equation}
In other word, a NE is a feasible strategy profile with the property that no single player can increase the utility by deviating from the strategy corresponding to the equilibrium, given the strategies of the other players. In the following subsections, we first analyze the existence and uniqueness for the NE of the formulated game ${\mathcal{G}}_{AF}$ and then develop a distributed algorithm for the links to achieve the NE.

\subsection{Existence of the NE}
The following theorem proposed in \cite{Glicksberg_AMS_1952} is usually adopted to verify the existence of the NE:
\begin{theorem}\label{thm:existence_NE}
A NE \emph{exists} in the game $\left\langle  {{\cal N},\{ {{\bf{{\cal Q}}}_n}\} ,\left\{ {{{\cal U}_n}\left( {{{\bf{x}}_n},{{\bf{x}}_{ - n}}} \right)} \right\}} \right\rangle $ if $\forall n \in {\cal N}$, ${{\bf{{\cal Q}}}_n}$ is a \emph{compact and convex} set; ${{{\cal U}_n}\left(  {\bf{q}}\right)}$ is continuous in ${\bf{q}}$ and \emph{quasi-concave} in ${{\bf{q}}_n}$, where ${\bf{q}} = \left({{{\bf{q}}_n},{{\bf{q}}_{ - n}}}\right)$.
\end{theorem}

After investigating the properties of the action sets and the utility functions for the formulated game ${\mathcal{G}}_{AF}$, we have the following proposition:
\begin{proposition}\label{prop:NE_existence_AF_game}
The utility function ${u_i^{AF}}\left( {{\rho _i},{\pmb \rho _{ - i}}} \right)$ is quasi-concave in $\rho_i$ for any $i \in \mathcal{N}$. Moreover, the formulated power splitting game ${\mathcal{G}}_{AF}$ for the pure AF network possesses at least one NE.
\end{proposition}
\begin{proof}
See Appendix \ref{append:prop1}.
\end{proof}

\subsection{Uniqueness of the NE}
Once the NE is ensured to exist, a natural question is whether it is unique. This is important not only for predicting the state of the network but also crucial for convergence issues.
In principle, the uniqueness of the NE can be analyzed by several methods, which has been summarized in \cite{Lasaulce_SPM_2009}. However, since the formulated game is not a convex game, most of the methodologies fail to apply except the approach of standard function \cite{Yates_JSAC_1995} because it only requires the best response function satisfies certain properties. To proceed, we first figure out the best response functions of the links (players) and have the following lemma:
\begin{lemma}\label{lemma:BR_AF}
Given a power splitting strategy profile $\pmb \rho$, the best response function of the link ${S_i} \to {R_i} \to {D_i}$ in the game ${\mathcal{G}}_{AF}$ can be expressed as
\begin{equation}\label{eq:BR_function_AF}
\begin{split}
{\mathcal B}_i^{AF}\left(\pmb \rho  \right) = \left\{ \begin{array}{l}
\frac{1}{2},\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;{\rm{if}}\;\left( {{X_i} + {Y_i}} \right)\left( {{W_i} + 1} \right) = {Z_i} \\
\frac{{\sqrt {{\left( {{X_i} + {Y_i} + 1} \right)\left( {{W_i} + 1} \right)}} }}{{\sqrt {\left( {{X_i} + {Y_i} + 1} \right)\left( {{W_i} + 1} \right)}  + \sqrt {Z_i +W_i+1} }},\;\;{\rm{if}}\;\left( {{X_i} + {Y_i}} \right)\left( {{W_i} + 1} \right) \ne {Z_i} \\
  \end{array} \right..
\end{split}
\end{equation}
\end{lemma}
\begin{proof}
See Appendix \ref{append:lemma_BR_AF}.
\end{proof}

We now define the vector function ${\pmb{\mathcal B}}^{AF}\left( \pmb \rho  \right) = \left[ {{{\mathcal B}_1^{AF}}\left( \pmb \rho  \right), \ldots ,{{\mathcal B}^{AF}_N}\left( \pmb \rho  \right)} \right]^T$. Then, according to the well-known fixed point theorem, the strategy profile ${\pmb \rho} ^*$ is a NE of the formulated game ${\mathcal{G}}_{AF}$ if and only if it is the fixed point of the function ${\pmb{\mathcal B}}^{AF}\left( \pmb \rho  \right)$ (i.e, ${\pmb{\mathcal B}}^{AF}\left( {\pmb \rho} ^*  \right) = {{\pmb \rho} ^* } $). Hence, the uniqueness for the NE of the formulated game is equivalent to that for the fixed point of the function ${\pmb{\mathcal B}}^{AF}\left( \pmb \rho  \right)$. Furthermore, it is shown in \cite{Yates_JSAC_1995} that the fixed point of the function ${\pmb{\mathcal B}}^{AF}\left( \pmb \rho  \right)$ is unique if ${\pmb{\mathcal B}}^{AF}\left( \pmb \rho  \right)$ is a \emph{standard} function. The standard function is defined as follows:
\begin{definition}
A function ${\bf{ f}}\left( \bf x  \right)$ is said to be standard if it satisfies the following properties for all $\bf x \ge0$:
\begin{itemize}
  \item \emph{Positivity}: ${\bf{f}}\left( \bf x \right) > \bf{0}$.
  \item \emph{Monotonicity}: If ${\bf x} \ge {{\bf x} ^\prime}$, then ${\bf{f}}\left( \bf x  \right) \ge {\bf{f}}\left( {\bf x}^\prime  \right)$.
  \item \emph{Scalability}: For all $\alpha >1 $, $\alpha {\bf{f}}\left( \bf x  \right)> {\bf{f}}\left( \alpha {\bf x}  \right)$.
\end{itemize}
Here, all the inequalities are componentwise.
\end{definition}

After investigating the properties of the best response functions given in Lemma \ref{lemma:BR}, we have the following proposition regarding the uniqueness of the NE:
\begin{proposition}\label{prop:NE_unique_AF}
The formulated game $\mathcal G_{AF}$ for the pure AF network always admits a unique NE.
\end{proposition}
\begin{proof}
See Appendix \ref{append:Prop_NE_unique_AF}.
\end{proof}

\subsection{Distributed Algorithm}\label{sec:algorithm_AF}
So far, we have proved that the formulated game ${\mathcal {G}}_{AF}$ always has a unique NE for any channel conditions and network topologies. However, this equilibrium is meaningful in practice only if one can develop an algorithm that is able to achieve such an equilibrium from non-equilibrium states. In this subsection, we propose a distributed and iterative algorithm with provable convergence to achieve the NE, in which the links update their power splitting ratios simultaneously. In addition, we discuss the practical implementation of the proposed algorithm.

\subsubsection{Algorithm Description}
Various kinds of distributed algorithms have been proposed to find the NE (see \cite{Lasaulce_book_2011} for more information). Here, we are interested in best response-based algorithms since we have obtained the best response functions of the formulated game. Relying on the derived best response function (\ref{eq:BR_function_AF}), we develop a distributed power splitting algorithm for the formulated game ${\mathcal {G}}_{AF}$, which is formally described in {\bf{Algorithm 1}}. In terms of the convergence of Algorithm 1, we have
\begin{proposition}\label{prop:convergence_alg_AF}
From any initial point, Algorithm 1 always converges to the unique NE of the formulated game $\mathcal G_{AF}$.
\end{proposition}
\begin{proof}
Since the best response vector function ${\pmb{\mathcal B}}^{AF}\left( \pmb \rho  \right)$ is standard (proved in Appendix \ref{append:Prop_NE_unique_AF}), the proof of this proposition follows with reference to \cite[Thm. 2]{Yates_JSAC_1995}.
\end{proof}

\begin{table}
\begin{center}
\begin{algorithm}[H]
%\algsetup{linenosize=\normalsize}
%\normalsize
%\textbf{Input:}$\quad$ Positive integer $\upsilon$.\\
%\textbf{Output:}$\quad$ Binary matrices $\boldsymbol G_{2,q}$, $q=1,2,\cdots,2^{\upsilon-1}$.\\
%\textbf{Steps:}
\begin{algorithmic}[1]
\small
\STATE Set ${t} = 0$ and each player (link) $i\in{\mathcal N}$ chooses a random power splitting ratio ${\rho}_i{\left(0\right)}$ from the feasible set ${\mathcal A}_i$.
%\STATE {\textbf {for}} ${t} = 0:{\rm{Number\_of\_Iteration}}-1$
\STATE If a suitable termination criterion is satisfied: $\rm{STOP}$.
\STATE Each link $i \in {\mathcal N}$ updates the power splitting ratio via executing
\begin{equation*}
%\footnotesize
\begin{split}
\rho_i(t+1) = {\mathcal{B}}_i^{AF}\left(\pmb \rho(t)\right).
\end{split}
\end{equation*}
%\STATE
%\begin{adjustwidth}{0.5cm}{0cm}
%The energy provider determines the value of $\gamma(t+1)$, and broadcasts that value as well as ${\bf{q}}_{\Sigma}{\left( {{t+1}} \right)} = \sum\nolimits_{n = 1}^N {{\bf{q}}_n{\left( {{t+1}} \right)}} $ to the consumers.
%\end{adjustwidth}
\STATE
%\begin{adjustwidth}{0.5cm}{0cm}
$t \leftarrow t + 1$; go to $\rm{STEP}$ 2.
%\end{adjustwidth}
%\STATE {\textbf {Until}} the termination criterion is satisfied.
\end{algorithmic}
\caption{: Distributed Power Splitting Algorithm for the Pure AF Network
}
\end{algorithm}
\end{center}
%\caption{Description of \textbf{Algorithm $1$} that is used to generate a series of full column rank binary matrices.}\label{fig:alg1}
\end{table}

\subsubsection{Implementation Discussion}
Note that the distributed nature of the above algorithm is based on modeling each whole link as a player. However, each link consists of three nodes (i.e., source, relay, and destination), which are geographically separated in practical networks. Thus, an efficient implementation of the proposed algorithm with the minimum information sharing should be designed.

In our design, the relay node is expected to be the link coordinator that undertakes the information collection and the best-response computation. Here, we assume that the energy consumed for the algorithm computations at the relay nodes are negligible compared with the harvested energy used for information forwarding. This assumption is valid with the rapid development of the low-power chips. Next, we aim to identify the information that is needed to collect or exchange for the implementation of the proposed algorithm. According the best response functions given in (\ref{eq:BR_function_AF}), the $i$th relay node needs to know the values of the parameters $X_i$, $Y_i$, $Z_i$, and $W_i$ defined in (\ref{eq:def_XYZW}). To this end, the $i$th relay node should perform the following tasks:
\begin{itemize}
  \item {\emph{Task 1}}: Measure the channel gains $g_{ii}$ and $h_{ii}$ (through training sent by the source $S_i$ and the destination $D_i$), acquire the transmission power $P_i$ from its source, and then calculate the value of $X_i$ based on these information.
  \item {\emph{Task 2}}: Measure\footnote{The measurement of the signal power can be performed by the radio scene analyzer \cite{Shi_TWC_2009}.} the power of its received signal, acquire the power of the received signal at the destination $D_i$ (through feedback from $D_i$), and then calculate the values of $Y_i$, $Z_i$, $W_i$.
  \item {\emph{Task 3}}: Calculate the optimal power splitting ratio $\rho_i$ based on (\ref{eq:BR_function_AF}).
\end{itemize}

Thus, the proposed algorithm requires no signaling between different links and only need a small amount of ``local" coordination among each link.




==> power_splitting_DF_network.tex <==
\section{Distributed Power Splitting Scheme for Pure DF Network}\label{sec:Pure_DF_Network}

In this section, we aim to find an efficient power splitting ratio profile for an alternative network scenario, where all the relay nodes adopt the DF relaying protocol. From the perspective of network utility maximization, the optimal power splitting ratio profile can be obtained through solving the following optimization problem:
\begin{equation}\label{eq:centralized_opt_DF}
\begin{array}{l}
\mathop {\max }\limits_{\pmb \rho}~ \sum\nolimits_{i = 1}^N {u_i^{DF}\left( {\pmb \rho}  \right)} \\
~~~~~{\rm{s}}{\rm{.t}}{\rm{.}}\;\;{\pmb \rho}  \in {\mathcal A}
\end{array},
\end{equation}
where ${u_i}^{DF}\left( {{\rho _i},{\pmb \rho _{ - i}}} \right) = \frac{1}{2}\min \left( {\log \left( {1 + \gamma _{i,1}^{DF}} \right),\log \left( {1 + \gamma _{i,2}^{DF}} \right)} \right)$ with $\gamma _{i,1}^{DF}$ and $\gamma _{i,2}^{DF}$ defined in (\ref{eq:DF_SNR_1st_hop}) and (\ref{eq:DF_SNR_2rd_hop}). Yet, it can be shown that the optimization problem in (\ref{eq:centralized_opt_DF}) is not only non-convex but also non-differentiable (the $\min$ operator). Thus, it cannot be efficiently solved even in a centralized manner. Motivated by this problem and analogous to Section \ref{sec:Pure_AF_Network}, we resort to the game-theoretical approach. More specifically, we consider that the links are selfish and they aim to maximize their individual utility by choosing the power splitting ratio. Mathematically, this will involve the $i$th link solving the following optimization problem
\begin{equation}\label{eq:DF_game_utility}
\begin{array}{l}
\mathop {\max }\limits_{{\rho _i}} \;\;\;{u_i^{DF}}\left( {{\rho _i},{\pmb \rho _{ - i}}} \right) \\
~~~~{\rm{s.t.}}\;\;\;{\rho _i} \in {{\mathcal A}_i}
\end{array}.
\end{equation}
Moreover, the power splitting problem for the considered pure DF network can be modeled by the following non-cooperative game:
\begin{itemize}
\item \emph{{Players}}: The $N$ S-R-D links.
\item \emph{{Actions}}: Each link determines its power splitting ratio $\rho_i \in {\mathcal{A}}_i$ to maximize the achievable rate for its own link.
\item \emph{{Utilities}}: The achievable rate ${u_i^{DF}}\left( {{\rho _i},{\pmb \rho _{ - i}}} \right)$ defined in (\ref{eq:utility_DF}).
\end{itemize}
For convenience, we denote the formulated non-cooperative game as
\begin{equation}\label{eq:game_DF}
{\mathcal{G}}_{DF} = \left\langle {\mathcal{N},\left\{ \mathcal{A}_i  \right\},\left\{{{u}_i^{DF}}\left( {{\rho_i},{{\pmb{\rho}}_{ -i}}} \right)\right\} }\right\rangle.
\end{equation}

In the following subsections, we first analyze the existence and uniqueness for the NE of the formulated game ${\mathcal{G}}_{DF}$ and then develop a distributed algorithm for the links to achieve the NE.

\subsection{Existence and Uniqueness of the NE}
After investigating the properties of the action sets and utility functions for the formulated game, we have the following proposition regarding the existence of the NE for the game ${\mathcal{G}}_{DF} $:
\begin{proposition}\label{prop:NE_existence_DF}
The formulated power splitting game ${\mathcal G}_{DF}$ possesses at least one NE.
\end{proposition}
\begin{proof}
See Appendix \ref{append:proof_NE_existence_DF}.
\end{proof}

When it comes to the uniqueness of the NE, most of the methodologies fail to apply except the approach of standard function \cite{Yates_JSAC_1995} due to the non-differentiability of the utility functions (the $\min$ operator). To proceed, we derive the best response functions of the links (players) in the game ${\mathcal G}_{DF}$ and have the following lemma:
\begin{lemma}\label{lemma:BR}
Given a power splitting strategy profile $\pmb \rho$, the best response function of the link ${S_i} \to {R_i} \to {D_i}$ in the game ${\mathcal G}_{DF}$ can be expressed as
\begin{equation}\label{eq:BR_function_DF}
\begin{split}
{{\mathcal B}_i^{DF}}\left(\pmb \rho  \right)&= \left[ {\left( {{X_i}{W_i} + {X_i} + {Y_i}{Z_i} + {Z_i}} \right) - } \right. \\
&\left. {\sqrt {{{\left( {{X_i}{W_i} + {X_i} - {Y_i}{Z_i} + {Z_i}} \right)}^2} + 4{Y_i}Z_i^2} } \right]/\left( {2{Y_i}{Z_i}} \right).
\end{split}
\end{equation}
\end{lemma}
\begin{proof}
See Appendix \ref{append:lemma_BR_function_DF}.
\end{proof}

We now define the vector function ${\pmb{\mathcal B}}^{DF}\left( \pmb \rho  \right) = \left[ {{{\mathcal B}_1^{DF}}\left( \pmb \rho  \right), \ldots ,{{\mathcal B}_N^{DF}}\left( \pmb \rho  \right)} \right]^T$. After investigating the properties of the function ${\pmb{\mathcal B}}^{DF}\left( \pmb \rho  \right)$, we have the following proposition regarding the uniqueness of the NE:
\begin{proposition}\label{prop:NE_unique}
The game ${\mathcal G}_{DF}$ always admits a unique NE.
\end{proposition}
\begin{proof}
See Appendix \ref{append:Prop_2}.
\end{proof}

\subsection{Distributed Algorithm}
Based on the best response function given in (\ref{eq:BR_function_DF}), we develop a distributed and iterative algorithm to achieve the NE of the formulated game in this subsection. The proposed algorithm is formally described in {\bf{Algorithm 2}}. In terms of the convergence of Algorithm 2, we have
\begin{proposition}\label{prop:convergence_alg_DF}
From any initial point, Algorithm 2 always converges to the unique NE of the formulated game ${\mathcal G}_{DF}$.
\end{proposition}
\begin{proof}
Since the best response vector function ${\pmb{\mathcal B}}^{DF}\left( \pmb \rho  \right)$ is standard (proved in Appendix \ref{append:Prop_2}), the proof of this proposition follows with reference to \cite[Thm. 2]{Yates_JSAC_1995}.
\end{proof}
Note that the practical implementation of Algorithm 2 can be analogous to that of the Algorithm 1 described in Section \ref{sec:algorithm_AF}.
\begin{table}
\begin{center}
\begin{algorithm}[H]
%\algsetup{linenosize=\normalsize}
%\normalsize
%\textbf{Input:}$\quad$ Positive integer $\upsilon$.\\
%\textbf{Output:}$\quad$ Binary matrices $\boldsymbol G_{2,q}$, $q=1,2,\cdots,2^{\upsilon-1}$.\\
%\textbf{Steps:}
\begin{algorithmic}[1]
\small
\STATE Set ${t} = 0$ and each player (link) $i\in{\mathcal N}$ chooses a random power splitting ratio ${\rho}_i{\left(0\right)}$ from the feasible set ${\mathcal A}_i$.
%\STATE {\textbf {for}} ${t} = 0:{\rm{Number\_of\_Iteration}}-1$
\STATE If a suitable termination criterion is satisfied: $\rm{STOP}$.
\STATE Each link $i \in {\mathcal N}$ updates the power splitting ratio via executing
\begin{equation*}
%\footnotesize
\begin{split}
\rho_i(t+1) = {\mathcal{B}}_i^{DF}\left(\pmb \rho(t)\right).
\end{split}
\end{equation*}
%\STATE
%\begin{adjustwidth}{0.5cm}{0cm}
%The energy provider determines the value of $\gamma(t+1)$, and broadcasts that value as well as ${\bf{q}}_{\Sigma}{\left( {{t+1}} \right)} = \sum\nolimits_{n = 1}^N {{\bf{q}}_n{\left( {{t+1}} \right)}} $ to the consumers.
%\end{adjustwidth}
\STATE
%\begin{adjustwidth}{0.5cm}{0cm}
$t \leftarrow t + 1$; go to $\rm{STEP}$ 2.
%\end{adjustwidth}
%\STATE {\textbf {Until}} the termination criterion is satisfied.
\end{algorithmic}
\caption{: Distributed Power Splitting Algorithm for the Pure DF Network
}
\end{algorithm}
\end{center}
%\caption{Description of \textbf{Algorithm $1$} that is used to generate a series of full column rank binary matrices.}\label{fig:alg1}
\end{table}



